Beyond Exact Gradients: Convergence of Stochastic Soft-Max Policy Gradient Methods with Entropy Regularization

Entropy regularization is an efficient technique for encouraging exploration and preventing a premature convergence of (vanilla) policy gradient methods in reinforcement learning (RL). However, the theoretical understanding of entropy-regularized RL algorithms has been limited. In this paper, we revisit the classical entropy regularized policy gradient methods with the soft-max policy parametrization, whose convergence has so far only been established assuming access to exact gradient oracles. To go beyond this scenario, we propose the first set of (nearly) unbiased stochastic policy gradient estimators with trajectory-level entropy regularization, with one being an unbiased visitation measure-based estimator and the other one being a nearly unbiased yet more practical trajectory-based estimator. We prove that although the estimators themselves are unbounded in general due to the additional logarithmic policy rewards introduced by the entropy term, the variances are uniformly bounded. We then propose a two-phase stochastic policy gradient (PG) algorithm that uses a large batch size in the first phase to overcome the challenge of the stochastic approximation due to the non-coercive landscape, and uses a small batch size in the second phase by leveraging the curvature information around the optimal policy. We establish a global optimality convergence result and a sample complexity of $\widetilde{\mathcal{O}}(\frac{1}{\epsilon^2})$ for the proposed algorithm. Our result is the first global convergence and sample complexity results for the stochastic entropy-regularized vanilla PG method.

==> sec/appe_SPG_online_part.tex <==
\subsection{Proof of Lemma \ref{lemma: Max Ent PG}}
\begin{proof}
\mynewred{The gradient \ref{eq: Maxent PG} follows from  Proposition 2 in \cite{cayci2021linear}. In particular, they consider the softmax parameterization with linear function approximation:
\begin{align*}
    \pi_\theta (a \mid s) = \frac{\exp({\theta^\top \phi_{s,a}}) }{ \sum_{a^\prime \mathcal{A}} \exp({\theta^\top \phi_{s,a^\prime}}) }
\end{align*}
Our tabular softmax parameterization setting is a special case by taking $\phi_{s,a} = e(s,a)  $ where $ e(s,a) \in \mathbb{R}^{|\mathcal{S}| |\mathcal{A}| }  $ is a vector where the $(s,a)$-th entry is equal to $1$ while all other entries equal to $0$.\\
The second part of the statement of Lemma \ref{lemma: Max Ent PG} holds due to the following simple algebra:
\begin{align*}
\left\|\frac{\partial V_\lambda^\theta(\rho)}{\partial \theta}\right\|  \leq& \frac{1}{1-\gamma} \max _{a, s}\left\|\nabla \log \pi_\theta(a \mid s)\right\| \\
&\times \max _s\left\|\sum_a \pi_\theta(a \mid s)\left[Q_\lambda^\theta(s, a)-\lambda \log \pi_\theta(a \mid s)\right]\right\| \\ 
 =&\frac{1}{1-\gamma} \max _{a, s}\left\|\nabla \log \pi_\theta(a \mid s)\right\| \times \max _s\left\|V_\lambda^\theta(s)\right\| \\
 & \leq \frac{2(\bar{r}+\lambda \log |\mathcal{A}|)}{(1-\gamma)^2} .\end{align*}
 }
\end{proof}


\subsection{Proof of Lemma \ref{lemma: unbias}}
\begin{proof}
We first show the unbiasedness of the Q-estimate, i.e., $\mathbb{E}\left[\hat{Q}^{\theta}_\lambda(s, a) \mid \theta, s, a\right]=Q^{\theta}_\lambda(s, a)$ for all $(s, a) \in \mathcal{S} \times \mathcal{A}$ and $\theta \in \mathbb{R}^{d}$. In particular, from the definition of $Q^{\theta}_\lambda(s, a)$, we have
\begin{align*}
& \mathbb{E}\left[\hat{Q}^{\theta}_\lambda(s, a) \mid \theta, s, a\right] \\
=&\mathbb{E}\left[r\left(s_{0}, a_{0}\right)+\sum_{h=1}^{H^{\prime}} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right)-\lambda \log{\pi_\theta(a_h|s_h)}\right) \right.\\
& \left.\hspace{6cm}\mid \theta, s_{0}=s, a_{0}=a\right] \\
=&\mathbb{E}\left[r\left(s_{0}, a_{0}\right)+\sum_{h=1}^{\infty} \mathbb{1}_{H^\prime\geq h\geq 0}\gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right)\right.\right.\\
& \left.\left.\hspace{3cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)  \mid \theta, s_{0}=s, a_{0}=a\right],
\end{align*}
where we have replaced $H^{\prime}$ by $\infty$ since we use the indicator function $\mathbb{1}$ such that the summand for $h \geq H^{\prime}$ is null. In addition, by the law of total expectation, we have
\begin{align} \label{eq: law of total expectation}
 &\mathbb{E}\left[\hat{Q}^{\theta}_\lambda(s, a) \mid \theta, s, a\right]\\ \nonumber=&\mathbb{E}_{H^\prime} \left[ \mathbb{E}_{\tau}\left[ r\left(s_{0}, a_{0}\right)+\sum_{h=1}^{\infty} \mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right) \right. \right.\right.\\
\nonumber &\left.\left.\left.\hspace{1.5cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)  \mid \theta, s_{0}=s, a_{0}=a , H^\prime\right]\right],
\end{align}
where the trajectory $\tau$ equal to $\{s_0,a_0,s_1,a_1,\ldots\}$.
The inner expectation over $\tau$ can be written as
\begin{align}\label{eq: inner expectation}
\nonumber \mathbb{E}_{\tau} & \left[r\left(s_{0}, a_{0}\right)+\sum_{h=1}^{\infty} \mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right)\right.\right.\\
\nonumber & \left.\left.\hspace{0.5cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right) \mid \theta, s_{0}=s, a_{0}=a , H^\prime\right] \\
\nonumber=& \sum_{\tau}\left[r\left(s_{0}, a_{0}\right)+\sum_{h=1}^{\infty} \mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right)\right.\right.\\
\nonumber & \left.\left.\hspace{0.5cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)\right]\cdot\mathbb{P}(\tau ) \left\mid\right. \theta, s_{0}=s, a_{0}=a , H^\prime\\
\nonumber =& r\left(s_{0}, a_{0}\right)+\sum_{\tau}\sum_{h=1}^{\infty}\left[ \mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right)\right.\right.\\
& \left.\left.\hspace{0.5cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)\right] \cdot\mathbb{P}(\tau ) \left\mid\right. \theta, s_{0}=s, a_{0}=a , H^\prime.
\end{align}
By the definition of the probability over the sample trajectory $\mathbb{P}(\tau )$, for every $h \in \{0,1,2,\ldots\}$, it holds that
\begin{align*}
&\left|\left( r\left(s_{h}, a_{h}\right)-\lambda \log{\pi_\theta(a_h|s_h)}\right) \cdot\mathbb{P}(\tau )\right|\\
=&\left| \left( r\left(s_{h}, a_{h}\right)-\lambda \log{\pi_\theta(a_h|s_h)}\right) \cdot \pi_\theta(a_h|s_h) \cdot \mathbb{P}(s_1|s_0,a_0)\right.\\
&\cdot \pi_\theta(a_1|s_1)\ldots \cdot\mathbb{P}(s_h|s_{h-1},a_{h-1})\cdot\mathbb{P}(s_{h+1}|s_{h},a_{h})\ldots\\
&\left.\mathbb{P}(s_{H^\prime}|s_{H^\prime-1},a_{H^\prime-1})\cdot  \cdot\pi_\theta(a_{H^\prime}|s_{H^\prime})\right|\\
\leq& \bar{r}+  \frac{\lambda}{e}.
\end{align*}
where the last inequality follows from $\mathbb{P}(s^\prime|s,a)\leq 1$, $\pi_\theta(a|s)\leq 1$ for all $s, s^\prime \in \mathcal{S}$ and $a\in \mathcal{A}$ together with $|x \log x |\leq \frac{1}{e}$ for $x\in [0,1]$. Thus, for each trajectory $\tau$ and $N>0$, we have
\begin{align} \label{eq: bound of each summand 1}
\nonumber &\sum_{h=1}^{N} \left[\mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right)-\lambda \log{\pi_\theta(a_h|s_h)}\right)\right] \cdot\mathbb{P}(\tau )\\
\leq& \frac{1}{1-\gamma^{1/2}}\left(\bar{r}+  \frac{\lambda}{e}\right).
\end{align}
Since left-hand side of \eqref{eq: bound of each summand 1} is  non-decreasing and the limit as $N\rightarrow\infty$ exists, by the Monotone Convergence Theorem, we can interchange the limit with the summation over the trajectory $\tau$ in \eqref{eq: inner expectation} as follows:
\begin{align}
\nonumber\mathbb{E}_{\tau}&\left[r\left(s_{0}, a_{0}\right)+\sum_{h=1}^{\infty} \mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right)\right.\right.\\
\nonumber & \left.\left.\hspace{2cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right) \mid \theta, s_{0}=s, a_{0}=a , H^\prime\right] \\
\nonumber=& r\left(s_{0}, a_{0}\right)+\sum_{h=1}^{\infty}\sum_{\tau}\left[ \mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right)\right.\right.\\
\nonumber & \left.\left.\hspace{1cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)\right]\cdot\mathbb{P}(\tau ) \left\mid\right. \theta, s_{0}=s, a_{0}=a , H^\prime\\
\nonumber=& r\left(s_{0}, a_{0}\right)+\sum_{h=1}^{\infty}\EE_{\tau} \left[\mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2}  \left( r\left(s_{h}, a_{h}\right)\right.\right.\\
\nonumber & \left.\left.\hspace{2cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)\mid \theta, s_{0}=s, a_{0}=a , H^\prime \right].
\end{align}
In addition, for every $N>0$, we have
\begin{align} \label{eq: bound of each summand 2}
\nonumber & \sum_{h=1}^{N}\EE_{\tau} \left[\mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2}  \left( r\left(s_{h}, a_{h}\right)-\lambda \log{\pi_\theta(a_h|s_h)}\right)\right.\\
\nonumber& \left. \mid \theta, s_{0}=s, a_{0}=a , H^\prime \right]+r\left(s_{0}, a_{0}\right)\\
\nonumber&\leq \gamma^{1 / 2}\sum_{h=0}^{\infty}\EE_{\tau} \left[\gamma^{(h+1) / 2}  \left( r\left(s_{h}, a_{h}\right)-\lambda \log{\pi_\theta(a_h|s_h)}\right) \right.\\
\nonumber & \left.\mid \theta, s_{0}=s, a_{0}=a , H^\prime \right]+r\left(s_{0}, a_{0}\right)\\
\nonumber&\leq r\left(s_{0}, a_{0}\right)+\gamma^{1 / 2}\EE_{s_1}\left[V_{\lambda,\gamma/2}^\theta(s_1)\mid s_0,a_0 \right]\\
\nonumber&\leq \bar{r}+\frac{\gamma/2(\bar{r}+\lambda \log |\mathcal{A}|)}{1-\gamma/2}\\
&\leq \frac{\bar{r}+\lambda \log |\mathcal{A}|}{1-\gamma/2},
\end{align}
where the third inequality is due to the boundedness of the enrtopy-regularized value function in Lemma \ref{lemma: bound of V and Q}. Furthermore, since \eqref{eq: bound of each summand 2} is non-decreasing and the limit as $N\rightarrow\infty$ exists, by the Monotone Convergence Theorem, we can interchange the limit with the outer-expectation over $H^\prime$ in \eqref{eq: law of total expectation} as follows:
\begin{align} \label{eq: unbias of Q hat}
\mathbb{E}&\left[\hat{Q}^{\theta}_\lambda(s, a) \mid \theta, s, a\right] \\
\nonumber=&r\left(s_{0}, a_{0}\right)+ \lim_{N\rightarrow \infty}\mathbb{E}_{H^\prime}\left[ \mathbb{E}_{\tau}\left[\sum_{h=1}^{N} \mathbb{1}_{H^\prime\geq h\geq 0} \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right) \right. \right. \right.\\
\nonumber & \left.\left.\left.\hspace{1cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)  \mid \theta, s_{0}=s, a_{0}=a , H^\prime\right]\right]\\
\nonumber=&r\left(s_{0}, a_{0}\right)+\lim_{N\rightarrow \infty}\sum_{h=1}^{N}\left[ \mathbb{E}_{\tau}\left[\mathbb{E}_{H^\prime}\left[ \mathbb{1}_{H^\prime\geq h\geq 0}\right] \gamma^{h / 2} \cdot\left( r\left(s_{h}, a_{h}\right) \right. \right. \right.\\
\nonumber & \left.\left.\left.\hspace{1cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)  \mid \theta, s_{0}=s, a_{0}=a \right]\right]\\
\nonumber=&r\left(s_{0}, a_{0}\right)+\lim_{N\rightarrow \infty}\sum_{h=1}^{N}\left[ \mathbb{E}_{\tau}\left[\gamma^{h} \cdot\left( r\left(s_{h}, a_{h}\right) \right. \right. \right.\\
\nonumber & \left.\left.\left.\hspace{1cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)  \mid \theta, s_{0}=s, a_{0}=a \right]\right]\\
\nonumber=&r\left(s_{0}, a_{0}\right)+\mathbb{E}_{\tau}\left[\sum_{h=1}^{\infty}\left[ \gamma^{h} \cdot\left( r\left(s_{h}, a_{h}\right) \right. \right. \right.\\
\nonumber & \left.\left.\left.\hspace{1cm}-\lambda \log{\pi_\theta(a_h|s_h)}\right)  \mid \theta, s_{0}=s, a_{0}=a \right]\right]\\
\nonumber=&{Q}^{\theta}_\lambda(s, a)
\end{align}
where we have also used the fact that $H^\prime$ is drawn independently from the trajectory $\tau$ in the first equality,  the fact that $H^\prime \sim \text{Geom}(1-\gamma^{1/2})$ and thus $\mathbb{E}_{H^\prime}\left[ \mathbb{1}_{H^\prime\geq h\geq 0}\right]=\gamma^{t/2}$ in the second equality, and the interchangeability between the limit and the summation over the trajectory $\tau$ in the third equality. This completes the proof of the unbiasedness of $\hat{Q}^{\theta}_\lambda(s, a)$.

% Similar logic allows us to establish that $\hat{V}^{\theta}_\lambda(s)$ is an unbiased estimate of $V^{\theta}_\lambda(s)$, i.e.,
% \begin{align*}
% &\mathbb{E}\left[\hat{V}^{\theta}_\lambda(s) \mid \theta, s\right] ={V}^{\theta}_\lambda(s), \quad \forall s \in \mathcal{S}, \ \theta \in \mathbb{R}^{d},
% \end{align*}
% where the expectation is taken along the trajectory as well as with respect to the random horizon $H^{\prime} \sim \text{Geom}\left(1-\gamma^{1/ 2}\right)$. Therefore, if $s^{\prime} \sim \mathbb{P}(\cdot \mid s, a)$ and $a^{\prime} \sim \pi_{\theta}\left(\cdot \mid s^{\prime}\right)$, we have
% \begin{align}\label{eq: unbias of A}
% \mathbb{E}\left[ \hat{A}^{\theta}_\lambda(s, a) \right]=\mathbb{E}\left[\hat{Q}^{\theta}_\lambda(s,a)-\lambda \log \pi_{\theta}(s\mid a)-\hat{V}^{\theta}_\lambda(s)\right]=A^{\theta}_\lambda(s, a)
% \end{align}
% That is, $\hat{A}^{\theta}_\lambda(s, a)$ is an unbiased estimate of the advantage function $A^{\theta}_\lambda(s, a)$.

Now, we are ready to show unbiasedness of the stochastic gradients $\hat{\nabla} V^\theta_\lambda(\rho)$. It follows from Lemma \ref{lemma: Max Ent PG} that
\begin{align*}
\begin{aligned}
 &\mathbb{E}[\hat{\nabla} V^\theta_\lambda(\rho) \mid \theta]\\
 =&\mathbb{E}_{H,\left(s_{H}, a_{H}\right)}\left\{\mathbb{E}_{H^{\prime},\left(s^\prime_{1: H^\prime}, a^\prime_{1: H^\prime} \right)}
\left[\hat{\nabla} V^\theta_\lambda(\rho) \right.\right.\\
\nonumber & \left.\left. \hspace{5cm}\mid \theta, s^\prime_0=s_{H}, a^\prime_0=a_H \right] \mid \theta\right\} \\
=&\mathbb{E}_{H,\left(s_{H}, a_{H}\right)}\left(\mathbb{E}_{H^{\prime},\left(s^\prime_{1: H^{\prime}}, a^\prime_{1: H^{\prime}}\right)}\left\{\frac{1}{1-\gamma} \nabla_\theta \log \pi_\theta (a^\prime_0|s^\prime_0) \right.\right.\\ &\left.\left.\left(\hat{Q}^{\theta}_\lambda(s^\prime_0, a^\prime_0)-\lambda \log \pi_{\theta}(a^\prime_0 \mid s^\prime_0) \right)  \mid \theta, s^\prime_0=s_{H}, a^\prime_0=a_H, \right\} \mid \theta\right) \\
=&\mathbb{E}_{H,\left(s_{H}, a_{H}\right)}\left(\frac{1}{1-\gamma} \nabla_\theta \log \pi_\theta (a_H|s_H) \mathbb{E}_{H^{\prime},\left(s^\prime_{1: H^{\prime}}, a^\prime_{1: H^{\prime}}\right)}\right.\\
& \left.\left\{\left(\hat{Q}^{\theta}_\lambda(s^\prime_0, a^\prime_0)-\lambda \log \pi_{\theta}(a^\prime_0 \mid s^\prime_0) \right)  \mid \theta, s^\prime_0=s_{H}, a^\prime_0=a_H, \right\} \mid \theta\right) \\
=&\mathbb{E}_{H,\left(s_{H}, a_{H}\right)}\left\{\frac{1}{1-\gamma} \nabla_\theta \log \pi_\theta (a_H|s_H) \right.\\
&\left.\left({Q}^{\theta}_\lambda(s_H, a_H)-\lambda \log \pi_{\theta}(a_H \mid s_H) \right) \mid \theta\right\}.
\end{aligned}
\end{align*}
where we have used \eqref{eq: unbias of Q hat} in the last equality.
By using the identity function $\mathbb{1}_{h=H}$, the above expression can be further written as
\begin{align} \label{eq: final interchange}
&\mathbb{E}[\hat{\nabla} V^\theta_\lambda(\rho) \mid \theta]\\
\nonumber=&\frac{1}{1-\gamma}  \mathbb{E}_{H,\left(s_{H}, a_{H}\right)}\left\{\sum_{h=0}^{\infty} \mathbb{1}_{h=H} \nabla_\theta \log \pi_\theta (a_H|s_H) \right.\\
\nonumber&\left.\left({Q}^{\theta}_\lambda(s_H, a_H)-\lambda \log \pi_{\theta}(a_H \mid s_H) \right) \mid \theta\right\}.
% \nonumber&=\frac{1}{1-\gamma}  \mathbb{E}_{H,\left(s_{H}, a_{H}\right)}\left\{\sum_{h=0}^{\infty} \mathbb{1}_{h=H} \left(\text{diag}(\pi_\theta)-\pi_\theta \pi_\theta^\top\right) \left({Q}^{\theta}_\lambda(s_H, a_H)-\lambda \log \pi_{\theta}(a_H \mid s_H) \right) \mid \theta\right\}.
\end{align}

Since for the softmax parameterization $\pi_\theta$, we have 
% $\nabla_\theta \log \pi_\theta=\text{diag}(\pi_\theta)-\pi_\theta \pi_\theta^\top \in \mathbb{R}^{|\mathcal{S}| |\mathcal{A}| \times |\mathcal{S}| |\mathcal{A}|}$ and $\nabla_\theta \log \pi_\theta(a_H|s_H)= $ is the column 
\begin{align*}
&\frac{\partial \log \pi_\theta(a_H|s_H)}{\partial {\theta_{s,a}}} = \\
&\begin{cases} 
-\pi_\theta(a|s) \pi_\theta(a_H|s_H), & (s,a)\neq(s_H,a_H),\\
\pi_\theta(a_H|s_H) -\pi_\theta(a_H|s_H) \pi_\theta(a_H|s_H), & (s,a)=(s_H,a_H).
\end{cases}
\end{align*}
Thus, the term $\sum_{h=0}^{\infty} \mathbb{1}_{h=H} \nabla_\theta \log \pi_\theta (a_H|s_H)$ $\left({Q}^{\theta}_\lambda(s_H, a_H)-\lambda \log \pi_{\theta}(a_H \mid s_H) \right)$ is uniformly bounded for every $N>0$ and non-decreasing with respect to $N$, we can interchange the limit and the expectation in \eqref{eq: final interchange} by the Monotone Convergence Theorem to obtain
\begin{align*} 
&\mathbb{E}[\hat{\nabla} V^\theta_\lambda(\rho) \mid \theta]\\
=&\sum_{h=0}^{\infty} \frac{\mathbb{P}(H=h)}{1-\gamma} \cdot \mathbb{E}_{H,\left(s_{H}, a_{H}\right)}\left\{  \nabla_\theta \log \pi_\theta (a_H|s_H)  \right.\\
& \left. \left({Q}^{\theta}_\lambda(s_H, a_H)-\lambda \log \pi_{\theta}(a_H \mid s_H) \right) \mid \theta\right\}\\
=&\sum_{h=0}^{\infty} \gamma^h\cdot \mathbb{E}_{\left(s_{h}, a_{h}\right)}\left\{ \nabla_\theta \log \pi_\theta (a_H|s_H)\right.\\
& \left. \left({Q}^{\theta}_\lambda(s_H, a_H)-\lambda \log \pi_{\theta}(a_H \mid s_H) \right) \right\}\\
=&\sum_{h=0}^{\infty} \gamma^h \sum_{s\in\mathcal{S}, a\in \mathcal{A}} \mathbb{P}(s_h=s, a_h=a|s_0\sim\rho, \theta) \nabla_\theta \log \pi_\theta (a|s)  \\
&\left({Q}^{\theta}_\lambda(s, a)-\lambda \log \pi_{\theta}(a \mid s) \right)\\
=& \sum_{s\in\mathcal{S}, a\in \mathcal{A}} \nabla_\theta \log \pi_\theta (a|s) \left({Q}^{\theta}_\lambda(s, a)-\lambda \log \pi_{\theta}(a \mid s) \right)\\
&\sum_{h=0}^{\infty}\gamma^h\mathbb{P}(s_h=s, a_h=a|s_0\sim\rho, \theta) \\
=&\frac{1}{1-\gamma} \EE_{s\sim d_{\rho}^{\pi_{\theta}}, a \sim  \pi_{\theta}(\cdot \mid s)} \left[\nabla_\theta \log \pi_\theta (a|s) \right.\\
\nonumber & \left. \left({Q}^{\theta}_\lambda(s, a)-\lambda \log \pi_{\theta}(a \mid s) \right)\right].
\end{align*}
where the second equality is due to the fact that $H\sim\text{Geom}(1-\gamma)$ and thus $\mathbb{P}(h=H)=(1-\gamma)\gamma^h$, and the forth equality is due to the linearity of the integral and the finiteness of the state and action spaces. 
This completes the proof of unbiasedness of $\hat{\nabla} V^\theta_\lambda(\rho)$.
\end{proof}

\subsection{Proof of Lemma \ref{lemma: bounded variance}}
\begin{proof}
We first note that the policy gradient estimator $\hat{\nabla} V^{\theta}_\lambda(\rho)$ can be decomposed as:
\begin{align*}
&\nabla_\theta \log \pi_\theta (a_H|s_H) \left(\hat{Q}^{\theta}_\lambda(s_H, a_H)-\lambda \log{\pi_\theta (s_H, a_H)} \right)\\
=& \nabla_\theta \log \pi_\theta (a_H|s_H) \left(\sum_{i=0}^{H^\prime} \gamma^{i/2} \left( r(s_i^\prime,a_i^\prime) -\lambda \log{\pi_\theta (a_i^\prime|s_i^\prime)} \right) \right),
% =&\sum_{i=0}^{H^\prime} \gamma^{i/2}  r(s_i^\prime,a_i^\prime) - \sum_{i=0}^{H^\prime} \gamma^{i/2} \lambda \log{\pi_\theta (a_i^\prime|s_i^\prime)} 
\end{align*}
where $H\sim \text{Geom}(1-\gamma), H^\prime \sim \text{Geom}(1-\gamma^1/2)$, $(s^H, a^H) \sim \nu^{\pi_\theta}_\rho (s,a), s_0^\prime=s_H, a_0^\prime=a_H$.
To streamline the presentation, we introduce the following notations:
\begin{align*}
    g_1(s_H,a_H)&=\sum_{i=0}^{H^\prime} \gamma^{i/2}r(s_i^\prime,a_i^\prime), \\ 
    % g_2(s_H)=\sum_{j=0}^{H^{\prime\prime}} \gamma^{j/2}r(s_j^{\prime\prime},a_j^{\prime\prime}),\\
    g_2(s_H,a_H)&=\sum_{i=0}^{H^\prime} \gamma^{i/2} \lambda \log{\pi_\theta (a_i^\prime|s_i^\prime)},  
    % g_4(s_H)=\sum_{j=0}^{H^{\prime\prime}}\gamma^{j/2} \lambda \log{\pi_\theta (a_j^{\prime\prime}|s_j^{\prime\prime})}.
\end{align*}
Then, the policy gradient estimator $\hat{\nabla} V^{\theta}_\lambda(\rho)$ can be decomposed as:
\begin{align*}
\hat{\nabla} V^{\theta}_\lambda(\rho)=\frac{1}{1-\gamma} \nabla_\theta \log \pi_\theta (a_H|s_H) \left( g_1(s_H,a_H)-g_2(s_H,a_H)\right).
\end{align*}
By the definition of the variance and the Cauchy-Schwarz inequality, we have
\begin{align*}
&\text{Var}(\hat{\nabla} V^{\theta}_\lambda(\rho))\\
=&\frac{\norm{\nabla_\theta \log \pi_\theta (a_H|s_H)}^2}{(1-\gamma)^2}\text{Var} \left( g_1(s_H,a_H)-g_2(s_H,a_H)\right)\\
\leq &\frac{2\norm{\nabla_\theta \log \pi_\theta (a_H|s_H)}^2}{(1-\gamma)^2}\left(\text{Var}\left( g_1(s_H,a_H)\right)\right.\\ &\left.+\text{Var}\left(g_2(s_H,a_H)\right)\right)\\
\leq &\frac{8}{(1-\gamma)^2}\left(\text{Var}\left( g_1(s_H,a_H)\right)+\text{Var}\left(g_2(s_H,a_H)\right)\right),
\end{align*}
where the last inequality follows from $\norm{\nabla_\theta \log \pi_\theta (a_H|s_H)}\leq 2$ \cite{ding2021global}.
Since $g_1(s,a)$ is uniformly bounded, i.e., $\norm{g_1(s,a)}\leq \frac{\bar{r}}{1-\gamma^{1/2}}$ for all $s \in\mathcal{S}, a\in\mathcal{A}$, we must have 
\begin{align*}
  \text{Var}\left(g_1(s_H,a_H)\right)  \leq \frac{\bar{r}^2}{(1-\gamma^{1/2})^2}.
\end{align*}

Then, it remains to prove the bounded variance of $g_2$. Firstly, it can be seen that
\begin{align*}
   \norm{g_2}^2\leq & \lambda^2 \left(\sum_{i=0}^{H^\prime} \gamma^{i/2} \log{\pi_\theta (a_i^\prime|s_i^\prime)}\right)^2\\
   = &\lambda^2 \left(\sum_{i=0}^{H^\prime} \gamma^{i/4}\gamma^{i/4}\log \pi_\theta(a_i^\prime|s_i^\prime))\right)^2\\
   \leq &\lambda^2 \left(\sum_{i=0}^{H^\prime} \gamma^{i/2}\right) \left(\sum_{i=0}^{H^\prime} \gamma^{i/2} \left(\log\pi_\theta(a_i^\prime|s_i^\prime))\right)^2\right)\\
\leq & \frac{\lambda^2}{1-\gamma^{1/2}} \left(\sum_{i=0}^{H^\prime} \gamma^{i/2} \left(\log\pi_\theta(a_i^\prime|s_i^\prime))\right)^2\right),
\end{align*}
where the second inequality is due to the Cauchy-Schwarz inequality.
By fixing the state action pair $(s_H,a_H)$ and the horizon $H^\prime$ for now and taking expectation of $g_2$ only over the sample trajectory $\tau^\prime=\{s^\prime_0,a^\prime_0,\ldots,s^\prime_H,a^\prime_H\}$, it holds that
\begin{align} \label{eq: expectation of g2 square}
\nonumber &\EE_{\tau^\prime \sim p(\tau^\prime|\theta)}\left[ \norm{g_2}^2\right]\\
\leq &\frac{\lambda^2}{1-\gamma^{1/2}}  \sum_{i=0}^{H^\prime} \gamma^{i/2} \EE_{\tau^\prime \sim p(\tau^\prime|\theta)}\left[ \left(\log\pi_\theta(a^\prime_i|s^\prime_i)\right)^2\right].
\end{align}
Since the realizations of $a_i^\prime$ and $s_i^\prime$ do not depend on the randomness in $s^\prime_{i+1}, a^\prime_{i+1}, \ldots, s^\prime_H$, we have
\begin{align*}
&\EE_{\tau^\prime \sim p(\tau^\prime|\theta)}\left[ \left(\log\pi_\theta(a_i^\prime|s_i^\prime)\right)^2\right]\\
=&\EE_{ s_1^\prime\sim p(\cdot|a_0^\prime,s_0^\prime) \ldots a_{H-1}^\prime \sim \pi_\theta(\cdot|s_{H-1}^\prime), s_{H}^\prime \sim p(\cdot|s_{H-1}^\prime,a_{H-1}^\prime)}\left[ \left(\log\pi_\theta(a_i^\prime|s_i^\prime)\right)^2\right]\\
=& \EE_{s^\prime_1\sim p(\cdot|a^\prime_0,s^\prime_0) \ldots a^\prime_i \sim \pi_\theta(\cdot|s_i^\prime)}\left[ \left(\log\pi_\theta(a_i^\prime|s_i^\prime)\right)^2\right] \\ 
=& \EE_{s_1^\prime\sim p(\cdot|a_0^\prime,s_0^\prime) \ldots s_{i}^\prime \sim p(\cdot|a_{i-1}^\prime,s_{i-1}^\prime)}\left[ \sum_{a_i^\prime \in \mathcal{A}}  \pi_\theta(a_i^\prime|s_i^\prime)\left(\log\pi_\theta(a_i^\prime|s_i^\prime)\right)^2\right].
\end{align*}

By checking the optimality conditions for the optimization problem
\begin{align} \label{eq: constrained log x squre}
    \max \ \sum_{i=1}^n x_i (\log{x_i})^2 \quad \text{such that }  \sum_{i=1}^n x_i=1,
\end{align}
it can be concluded that  the maximizer for the constrained problem \eqref{eq: constrained log x squre} is $x_1=x_2=\ldots=x_n=\frac{1}{n}$ and the maximum solution is $(\log{n})^2$. 

Thus, we have $ \sum_{a_h \in \mathcal{A}}  \pi_\theta(a_h|s_h)\left(\log\pi_\theta(a^i_h|s^i_h)\right)^2 \leq (\log |\mathcal{A}|)^2$ and 
\begin{align*} 
&\EE_{\tau^\prime \sim p(\tau^\prime|\theta)}\left[ \left(\log\pi_\theta(a^i_h|s^i_h)\right)^2\right]\\
\leq & \EE_{s_0 \sim \rho, a_0 \sim \pi_\theta(\cdot|s_0), s_1\sim p(\cdot|a_0,s_0) \ldots s_{h} \sim p(\cdot|a_{h-1},s_{h-1})}\left[(\log |\mathcal{A}|)^2\right]\\
=&(\log |\mathcal{A}|)^2.
\end{align*}
By substituting the above inequality into \eqref{eq: expectation of g2 square},  we obtain that 
\begin{align*}
\EE_{\tau^\prime \sim p(\tau^\prime|\theta)}\left[ \norm{g_2}^2\right]\leq &\frac{\lambda^2}{1-\gamma^{1/2}}  \sum_{i=0}^{H^\prime} \gamma^{i/2} \EE_{\tau^\prime \sim p(\tau^\prime|\theta)}\left[ \left(\log\pi_\theta(a^\prime_i|s^\prime_i)\right)^2\right]\\
\leq & \frac{ (\lambda\log |\mathcal{A}|)^2}{1-\gamma^{1/2}}  \sum_{i=0}^{H^\prime} \gamma^{i/2} \\
\leq & \frac{ (\lambda\log |\mathcal{A}|)^2}{(1-\gamma^{1/2})^2},
\end{align*}
for every $H^\prime>0$.
By taking expectation of $g_2$ over the state action pair $(s_H,a_H)$ and the horizon $H^\prime$, it yields that
\begin{align*}
\EE\left[ \norm{g_2}^2\right]
\leq & \frac{ (\lambda\log |\mathcal{A}|)^2}{(1-\gamma^{1/2})^2},
\end{align*}
which further implies that $\text{Var}\left[ \norm{g_2}^2\right]
\leq  \frac{ (\lambda\log |\mathcal{A}|)^2}{(1-\gamma^{1/2})^2}$.
This completes the proof.
\end{proof}

\subsection{Proof of Lemma \ref{lemma:bias of truncation}}
\begin{proof}
To simplify the notation, we define $\Tilde{r}_{j,\theta}^\lambda \coloneqq r_{j}(s_{j},a_{j})-\lambda\log \pi_\theta(a_{j}|s_{j})$
By definition, we have
\begin{align*}
&\EE[\hat{\nabla} V^{\theta,H}_\lambda(\rho)]-{\nabla} V^{\theta}_\lambda(\rho)\\
% =&\EE\left[ \sum_{h=0}^{\infty} \nabla \log \pi_\theta(a_h|s_h)\left(\sum_{j=h}^{\infty} \gamma^{j} \left(r_{j}(s_{j},a_{j})-\lambda\log \pi_\theta(a_{j}|s_{j}) \right)\right)\right.\\
% -&\left.\sum_{h=0}^{H-1} \nabla \log \pi_\theta(a_h|s_h)\left(\sum_{j=h}^{H-1} \gamma^{j} \left(r_{h}(s_{j},a_{j})-\lambda\log \pi_\theta(a_{j}|s_{j}) \right)\right)\right]\\
=&\EE\left[\sum_{h=0}^{H-1} \nabla \log \pi_\theta(a_h|s_h)\left(\sum_{j=H}^{\infty} \gamma^{j}\Tilde{r}_{j,\theta}^\lambda\right)\right.\\
+&\left.\sum_{h=H}^{\infty} \nabla \log \pi_\theta(a_h|s_h)\left(\sum_{j=h}^{\infty} \gamma^{j}\Tilde{r}_{j,\theta}^\lambda\right)\right]
% &\left.+ \lambda  \sum_{h=H}^{\infty}-\gamma^t\nabla \log \pi_\theta(a_h,s_h) \right]\\ 
\end{align*}
Then, by the Cauchy-Schwarz inequality and the triangle inequality, we obtain
\begin{align*}
& \norm{\EE[\hat{\nabla} V^{\theta,H}_\lambda(\rho)]-{\nabla} V^{\theta}_\lambda(\rho)}_2\\
% \leq&\norm{\EE\left[ \sum_{h=0}^{H-1} \nabla \log \pi_\theta(a_h|s_h)\left(\sum_{j=H}^{\infty} \gamma^{j} \left(r_{j}(s_{j},a_{j})-\lambda\log \pi_\theta(a_{j}|s_{j}) \right)\right)\right]}\\
% &+\norm{\EE\left[\sum_{h=H}^{\infty} \nabla \log \pi_\theta(a_h|s_h)\left(\sum_{j=h}^{\infty} \gamma^{j} \left(r_{j}(s_{j},a_{j})-\lambda\log \pi_\theta(a_{j}|s_{j}) \right)\right)\right]}\\
\leq&\EE\left[ \sum_{h=0}^{H-1} \norm{\nabla \log \pi_\theta(a_h|s_h)}\left(\sum_{j=H}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda \right)\right]\\
&+\EE\left[\sum_{h=H}^{\infty} \norm{\nabla \log \pi_\theta(a_h|s_h)}\left(\sum_{j=h}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda \right)\right].
% &+\EE\left[\lambda  \sum_{h=H}^{\infty}\gamma^t \norm{\nabla \log \pi_\theta(a_h,s_h)}\right]\\
\end{align*}
Since $\norm{\nabla \log\pi_\theta(a|s)}_2\leq 2$ for all $\theta \in \mathbb{R}^{|\mathcal{S}||\mathcal{A}|}$, it holds that 
\begin{align}
\nonumber & {\EE[\hat{\nabla} V^{\theta,H}_\lambda(\rho)]-{\nabla} V^{\theta}_\lambda(\rho)}_2\\
\leq&2\EE\left[ \sum_{h=0}^{H-1}\left(\sum_{j=H}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda\right)\right] \label{eq: bias 1}\\
&+2\EE\left[\sum_{h=H}^{\infty} \left(\sum_{j=h}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda\right)\right] \label{eq: bias 2}.
% &+2\EE\left[\lambda  \sum_{h=H}^{\infty}\gamma^t\right]. \label{eq: bias 3}
\end{align}
For the term in \eqref{eq: bias 1}, we can rewrite it as
\begin{align*}
&2\EE_{\tau^\infty}\left[ \sum_{h=0}^{H-1}\left(\sum_{j=H}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda\right)\right]=\sum_{\tau^\infty} \left[ \sum_{h=0}^{H-1}\left(\sum_{j=H}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda\right)\right] \cdot \mathbb{P}(\tau^\infty)
\end{align*}
Since left-hand side of the above equation is  non-decreasing and the limit as $N\rightarrow\infty$ exists, by the the Monotone Convergence Theorem, we can interchange the limit with the summation over the trajectory $\tau^\infty$ in \eqref{eq: bias 1} as follows:
\begin{align*}
&2\EE_{\tau^\infty}\left[ \sum_{h=0}^{H-1}\left(\sum_{j=H}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda\right)\right]\\
&=2 \sum_{h=0}^{H-1}\left(\sum_{j=H}^{\infty} \gamma^{j}\EE_{\tau^\infty}\left[ r_{j}(s_{j},a_{j})-\lambda\log \pi_\theta(a_{j}|s_{j}) \right]\right).
\end{align*}
Due to $- \sum_a \pi(a|s)\cdot \log \pi(a|s)\leq \log |\mathcal{A}|$, the term in \eqref{eq: bias 1} can be upper bounded as
\begin{align*}
&2\EE_{\tau^\infty}\left[ \sum_{h=0}^{H-1}\left(\sum_{j=H}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda\right)\right]\leq 2(\bar{r}+\lambda\log{|\mathcal{A}|}) \sum_{h=0}^{H-1}\left(\sum_{j=H}^{\infty} \gamma^{j}\right)\\
&\leq  \frac{2(\bar{r}+\lambda\log{|\mathcal{A}|})H \gamma^H}{1-\gamma}.
\end{align*}

Similarly, we can interchange  the limit with the summation over the trajectory $\tau^\infty$ in \eqref{eq: bias 2} and upper bound it as
\begin{align*}
2\EE\left[\sum_{h=H}^{\infty} \left(\sum_{j=h}^{\infty} \gamma^{j} \Tilde{r}_{j,\theta}^\lambda\right)\right]\leq & 2(\bar{r}+\lambda\log{|\mathcal{A}|}) \sum_{h=H}^{\infty}\sum_{j=h}^{\infty} \gamma^{j}\\
\leq& \frac{ 2(\bar{r}+\lambda\log{|\mathcal{A}|})\gamma^H}{(1-\gamma)^2}.
\end{align*}
% For the term in  \eqref{eq: bias 3}, it can be easily bounded as 
% \begin{align*}
%     2\EE\left[\lambda  \sum_{h=H}^{\infty}\gamma^t\right] \leq \frac{2\lambda \gamma^H}{1-\gamma}.
% \end{align*}
Combining the above two inequalities, we have
\begin{align*}
&\norm{\EE[\hat{\nabla} V^{\theta,H}_\lambda(\rho)]-{\nabla} V^{\theta}_\lambda(\rho)}_2\\
\leq& \frac{ 2(\bar{r}+\lambda\log{|\mathcal{A}|})\gamma^H}{(1-\gamma)} \left(H+\frac{1}{1-\gamma}\right).
\end{align*}
This completes the proof.
\end{proof}



==> sec/appex_asym_convergence.tex <==
\section{Helpful lemma for Lemma \ref{thm: high complexity global convergence}} \label{sec: proof for thm: high complexity global convergence}


% \begin{lemma} \label{lemma: delta under tau >T}
% Let $e_t=\nabla V_\lambda^{\theta_t}(\rho)-u_t$, where $u_t=\frac{1}{B} \sum_{i=1}^B\hat{\nabla} V_\lambda^{\theta_t,i}(\rho)$ and $\hat{\nabla} V_\lambda^{\theta_t,i}(\rho)$ is an unbiased estimator of $\nabla V_\lambda^{\theta_t}(\rho)$. If $\eta_t=\eta\leq \frac{1}{2L}$,  then
% \begin{align*}
% \EE[D(\theta_T) \mathbf{1}_{\tau>T}]\leq & \left(1-\frac{\eta C^0_\delta}{8}\right)^{T-1} D(\theta_1)+ \frac{5 \sigma^2}{8C^0_\delta B}.
% \end{align*}
% \end{lemma}


% \begin{lemma}\label{lemma: prob tau <T}
% Let $e_t=\nabla V_\lambda^{\theta_t}(\rho)-u_t$, where $u_t=\frac{1}{B} \sum_{i=1}^B\hat{\nabla} V_\lambda^{\theta_t,i}(\rho)$ and $\hat{\nabla} V_\lambda^{\theta_t,i}(\rho)$ is an unbiased estimator of $\nabla V_\lambda^{\theta_t}(\rho)$. Then, it holds that 
% \begin{align*}
% \mathbb{P}(\tau \leq T )\leq & \frac{ \delta \cdot\eta\cdot T\cdot (1+\eta L)^{T-1}\cdot{\sigma}  }{\bar{\Delta} B}.
% \end{align*}
% \end{lemma}





==> sec/appex_pilowerbound_whp.tex <==
\section{Helpful lemmas for Lemma \ref{lemma: pi lower bound high prob}}\label{sec: proof of Lemma pi lower bound high prob}
%  We first introduce some useful results before proceeding with the proof. 

% \begin{lemma}\label{lemma: D t+1 and D t}
% Suppose that $\{\theta_t\}$ is generated by Algorithm \ref{alg:unbiased PG} with $0<\eta_t\leq\frac{(1-\gamma)^3}{16\bar{r}+\lambda(8+16\log |\mathcal{A}|) }$ for all $t\geq 1$. We have
% \begin{align} \label{eq: D t+1 and D t}
%  D(\theta_{t+1})
%     \leq & \left(1-\frac{\eta_t C(\theta_t)}{4} \right)D(\theta_{t})-
%     \frac{\eta_t}{2}\xi_t+\frac{\eta_t}{4}\norm{e_t}_2^2,
% \end{align}
% where $\xi_t=\inner{e_t}{{\nabla}V^{\theta_t}_\lambda(\rho)}$ and $e_t=\hat{\nabla}V_\lambda^{\theta_t}(\rho)-{\nabla}V_\lambda^{\theta_t}(\rho)$.
% \end{lemma}


% \begin{lemma}\label{lemma: three claims}
%  Let $\pi_{\theta^*}$ be the optimal policy. Then, for all $n\in\{1,2, \ldots\}$, the following statements hold: 
%  \begin{enumerate}
%      \item $\Omega_{n+1} \subseteq \Omega_{n}$ and $E_{n+1} \subseteq E_{n}$.
%      \item $E_{n-1} \subseteq \Omega_{n}$.
%      \item Consider the ``large noise'' event
% $$
% \begin{aligned}
% \tilde{E}_{n} & \equiv E_{n-1} \backslash E_{n}=E_{n-1} \cap\left\{R_{n}>\varepsilon\right\} \\
% &=\left\{R_t \leq \varepsilon \text { for all } t=1,2, \ldots, n-1 \text { and } R_{n}>\varepsilon\right\}
% \end{aligned}
% $$
% and let $\tilde{R}_{n}=R_{n} \mathbb{1}_{E_{n-1}}$ denote the cumulative error subject to the noise being ``small'' until time $n$. Then,
% \begin{align}\label{eq: third argument}
%     \mathbb{E}\left[\tilde{R}_{n}\right] \leq \mathbb{E}\left[\tilde{R}_{n-1}\right]+G^2\sigma^2\eta_n^2+\frac{\eta_n \sigma^2}{4B}-\varepsilon \mathbb{P}\left(\tilde{E}_{n-1}\right).
% \end{align}
% % where $G=\frac{2(\bar{r}+\lambda \log |\mathcal{A}|)}{(1-\gamma)^2}$.
% By convention, we write $\tilde{E}_{0}=\varnothing$ and $\tilde{R}_{0}=0$.
%  \end{enumerate}
% \end{lemma}


% \begin{lemma}\label{lemma: En high prob}
% Consider an arbitrary  tolerance level $\delta>0$. If Algorithm \ref{alg:unbiased PG} is run with a step-size schedule of the form $\eta_t=1 /(t+t_0)$ for some sufficiently large $m>0$ and a batch size schedule $B_t\geq \frac{1}{\eta_t}$, we have
% $$
% \mathbb{P}\left(E_{n}\right) \geq 1-\delta \quad \text { for all } n=1,2, \ldots
% $$
% \end{lemma}




% \subsection{Proof of Theorem \ref{thm: convergence rate}} \label{sec: Proof of Theorem thm: convergence rate}
% % \begin{proposition}[Lemma 1 in \cite{Chung1954}] \label{prop: Lemma 1 in Chung1954}
% % Let $a_{t}, t=1,2, \ldots$, be a non-negative sequence such that
% % $$
% % a_{t+1} \leq\left[1-\frac{P}{(t+t_0)}\right] a_{n}+\frac{R}{(t+t_0)^{2}}
% % $$
% % where $P>1, R>0$. Then, we have
% % $$
% % a_{t} \leq \frac{R}{P-1} \frac{1}{t}+o\left(\frac{1}{t}\right).
% % $$
% % \end{proposition}
% % \subsubsection{Proof of Theorem \ref{thm: convergence rate}}

% \begin{proof}
% % We first define
% % \begin{align}\label{eq: definition of Omega alpha t}
% %     \Omega_{\alpha,n}=\left\{\min_{s,a} \pi_{\theta_t}(a|s)\geq (1-\alpha) \min_{s,a} \pi_{\theta^*}(a|s), \ \text { for all } t=1,2, \ldots,n\right\}.
% % \end{align}
% From Lemma \ref{lemma: D t+1 and D t}, we know
% \begin{align} 
% D(\theta_{t+1}) \mathbb{1}_{\Omega_{\alpha, t}}
%     \leq & \left(1-\frac{\eta_t C(\theta_t)}{4} \right)D(\theta_{t})\mathbb{1}_{\Omega_{\alpha, t}}-
%     \frac{\eta_t}{2}\xi_t\mathbb{1}_{\Omega_{\alpha, t}}+\frac{\eta_t}{4}\norm{e_t}_2^2\mathbb{1}_{\Omega_{\alpha, t}},
% \end{align}
% where $\xi_t=\inner{e_t}{{\nabla}V^{\theta_t}_\lambda(\rho)}$. When the event $\Omega_{\alpha, t}$ occurs, we have $C(\theta_t)\geq C_\alpha$ where
% \begin{align*}
%     C_\alpha\coloneqq\frac{2\lambda}{|\mathcal{S}|} \min_{s} \rho(s) (1-\alpha)^2\min_{s,a} \pi_{\theta^*}(a|s)^2 \norm{\frac{d_{\rho}^{\pi_\lambda^\ast}}{\rho}}_\infty^{-1}>0.
% \end{align*}
% % Then, for any given $\eta$, we can choose $t_0$ sufficiently large so that $\inf_t\left(1-\frac{\eta_t C_\alpha}{4} \right)>0$. Moreover, 
% By taking the expectation, we can obtain
% \begin{align*}
% \EE \left[ -\frac{\eta_t}{2}\xi_t\mathbb{1}_{\Omega_{\alpha, t}}+\frac{\eta_t}{4}\norm{e_t}_2^2\mathbb{1}_{\Omega_{\alpha, t}} \right]=&\EE \left[\mathbb{1}_{\Omega_{\alpha, t}}\EE \left[ -\frac{\eta_t}{2}\xi_t+\frac{\eta_t}{4}\norm{e_t}_2^2 \Big\mid \mathcal{F}_t\right]\right]\\
% =&\EE \left[\mathbb{1}_{\Omega_{\alpha, t}}\EE \left[ \frac{\eta_t}{4}\norm{e_t}_2^2 \Big\mid \mathcal{F}_t\right]\right]\\
% \leq & \frac{\eta_t \sigma^2}{4B},
% \end{align*}
% where the first equality is due to the fact that $\Omega_{\alpha, t}$ is deterministic conditioning on $\mathcal{F}_t$, 
% second equality is due to the unbiasedness of $\xi_t$ conditioning on $\mathcal{F}_t$ and the first inequality is due to \eqref{eq: third term bound}.
% Therefore,
% \begin{align*}
%   \EE[ D(\theta_{t+1})\mathbb{1}_{\Omega_{\alpha, t}}]
%     \leq &\left(1-\frac{\eta_t C_\alpha}{4}\right)\EE\left[ D(\theta_{t})\mathbb{1}_{\Omega_{\alpha, t}}\right]+\frac{\eta_t \sigma^2}{4B}.
% \end{align*}

% % For any given $T$, we have $B>\frac{1}{\eta_t}$ for every $t=1,2,.\ldots,T$. Thus,
% % \begin{align*}
% %   \EE[ D(\theta_{t+1})\mathbb{1}_{\Omega_{\alpha, t}}]
% %     \leq &\left(1-\frac{\eta_t C_\alpha}{4}\right)\EE\left[ D(\theta_{t})\mathbb{1}_{\Omega_{\alpha, t}}\right]+\frac{\eta_t^2 \sigma^2}{4}\\
% %     = &\left(1-\frac{\eta C_\alpha}{4(t+t_0)}\right)\EE\left[ D(\theta_{t})\mathbb{1}_{\Omega_{\alpha, t}}\right]+\frac{\eta^2 \sigma^2}{4(t+t_0)^2}.
% % \end{align*}

% % By choosing $\eta$ large enough such that $\eta>\frac{4}{C_\alpha}$, it follows from Proposition \ref{prop: Lemma 1 in Chung1954} that 
% % \begin{align*}
% %     \EE[ D(\theta_{t+1})\mathbb{1}_{\Omega_{\alpha, t}}]\leq \frac{\eta^2\sigma^2}{(\eta C_\alpha-4)t} +o(\frac{1}{t}).
% % \end{align*}
% Arguing inductively yields that
% \begin{align*}
%     \EE[D(\theta_{t+1})\mathbb{1}_{\Omega_{\alpha, t}}] \leq & \prod_{i=1} \left(1-\frac{\eta_i C_\alpha}{4}\right) \Delta_1 +\sum_{i=1}\left(1-\frac{\eta_i C_\alpha}{4}\right)^i\frac{\eta_i \sigma^2}{4B} \\
%     \leq & \prod_{i=1} \left(1-\frac{\eta_i C_\alpha}{4}\right) \Delta_1 +\sum_{i=1}\frac{\eta_i \sigma^2}{4B}.
% \end{align*}
% By setting $t+1=T$ and taking $\eta_i=\frac{4}{C_\alpha (i+t_0)}$, we obtain that
% \begin{align*}
% \EE[D(\theta_{T})\mathbb{1}_{\Omega_{\alpha, {T-1}}}]\leq & \prod_{i=1}^{T-1} \left(1-\frac{\eta_i C_\alpha}{4}\right) \Delta_1 +\sum_{i=1}^{T-1}\frac{\eta_i \sigma^2}{4B}\\
% \leq& \prod_{i=1}^{T} \left(1-\frac{\eta_i C_\alpha}{4}\right) \Delta_1 +\sum_{i=1}^{T}\frac{\eta_i \sigma^2}{4B}\\
% = & \prod_{i=1}^{T} \left(\frac{i+t_0-1}{i+t_0}\right) \Delta_1 +\frac{\sigma^2}{C_\alpha  B}\sum_{i=1}^{T}\frac{1}{i+t_0}\\
% \leq &\frac{t_0}{T+t_0} \Delta_1 +\frac{\sigma^2\ln{(T+t_0)}}{B C_\alpha}.
% \end{align*}

% Since $\Omega_{\alpha,T} \subseteq \Omega_{\alpha, t}$ for all $t=1,2,\ldots, T$. it follows that
% \begin{align*}
%     \EE[ D(\theta_{T})\mathbb{1}_{\Omega_{\alpha, T}}]\leq  &\frac{t_0}{T+t_0} \Delta_1 +\frac{\sigma^2\ln{(T+t_0)}}{B C_\alpha}.
% \end{align*}
% Then, the claim of the theorem follows by noting that
% \begin{align*}
% \EE[ D(\theta_{T})\mid {\Omega_{\alpha, T}}] \leq& \frac{\EE[ D(\theta_{T})\mathbb{1}_{\Omega_{\alpha, T}}]}{\mathbb{P}(\Omega_{\alpha, T})} \\
% \leq  &\frac{t_0}{(T+t_0)(1-\delta)} \Delta_1 +\frac{\sigma^2\ln{(T+t_0)}}{B(1-\delta) C_\alpha}.
% \end{align*}

% By the law of total probability and the Markov inequality, we obtain that
% \begin{align*}
% \mathbb{P}(D(\theta_{T}) \geq \epsilon) =  &    \mathbb{P}(D(\theta_{T}) \geq \epsilon \mathbb{1}_{\Omega_{\alpha, T}})+\mathbb{P}(D(\theta_{T}) \geq \epsilon \mathbb{1}_{\Omega_{\alpha, T}}^c)\\
% =  &    \mathbb{P}(D(\theta_{T}) \geq \epsilon \mid {\Omega_{\alpha, T}})\mathbb{P}( \Omega_{\alpha, T})+\mathbb{P}(D(\theta_{T}) \geq \epsilon \mid \Omega_{\alpha, T}^c)\mathbb{P}( \Omega_{\alpha, T}^c)\\
% \leq & \frac{\EE[D(\theta_{T})\mid {\Omega_{\alpha, T}}]}{\epsilon}\mathbb{P}( \Omega_{\alpha, T})+\mathbb{P}(D(\theta_{T}) \geq \epsilon \mathbb{1}_{\Omega_{\alpha, T}}^c)\mathbb{P}( \Omega_{\alpha, T}^c)\\
% \leq & \frac{\EE[D(\theta_{T})\mathbb{1}_{\Omega_{\alpha, T}]}}{\epsilon}+\delta\\
% \leq &\frac{t_0}{(T+t_0)\epsilon} \Delta_1 +\frac{\sigma^2\ln{(T+t_0)}}{B C_\alpha \epsilon}+\delta.
% \end{align*}
% % where the third inequality holds due to Lemma \ref{lemma: pi lower bound high prob} and the last inequality holds due to the first claim in Theorem \ref{thm: asym global convergence}. 

% To guarantee that $\mathbb{P}(D(\theta_{T}) \geq \epsilon) \leq \mathcal{O}(\delta)$, it suffices to have
% \begin{align*}
% T\geq \frac{t_0\Delta_1}{\delta\epsilon}-t_0, \quad B\geq \frac{\sigma^2\ln(T+t_0)}{C_\alpha \delta  \epsilon}.
% \end{align*}
% Thus, the total sample complexity is $T\cdot B=\tilde{\mathcal{O}}(\frac{1}{ \epsilon^2})$. This completes the proof.
% \end{proof}


